Accessing Higher Dimensions for Unsupervised Word Translation

The striking ability of unsupervised word translation has been demonstrated with the help of word vectors / pretraining; however, they require large amounts of data and usually fails if the data come from different domains. We propose coocmap, a method that can use either high-dimensional co-occurrence counts or their lower-dimensional approximations. Freed from the limits of low dimensions, we show that relying on low-dimensional vectors and their incidental properties miss out on better denoising methods and useful world knowledge in high dimensions, thus stunting the potential of the data. Our results show that unsupervised translation can be achieved more easily and robustly than previously thought -- less than 80MB and minutes of CPU time is required to achieve over 50\% accuracy for English to Finnish, Hungarian, and Chinese translations when trained on similar data; even under domain mismatch, we show coocmap still works fully unsupervised on English NewsCrawl to Chinese Wikipedia and English Europarl to Spanish Wikipedia, among others. These results challenge prevailing assumptions on the necessity and superiority of low-dimensional vectors, and suggest that similarly processed co-occurrences can outperform dense vectors on other tasks too.

==> junk.tex <==

\subsection{Word substitution cipher}
In this setting, each word is substituted by a symbol, and the \emph{decipherment} task
is to recover word identities after seeing some amount of data and given a model of the original data.
% Some properties of the problem is well-understood since \cite{shannon1949comm} and some early work \cite{knight-1999-decoding, ravi-knight-2011-deciphering} explicitly considers word-substitution.
For a vocabulary size of $V$, there are $k = V!$ possible word substitution ciphers.
Shannon's theory of unicity \citep{shannon1949comm} tells us that we need a sample size $N$ such that $(H_0 - H) N - \log k > 0$ to successfully solve a \emph{random} cipher and establishes the relationship between the redundancy $H_0 - H$ and the difficulty of solving the cipher.
In this analysis, there are $S = \exp(N H)$ high probability (i.e. typical) data samples of length $N$,
$T = \exp(N H_0) $ total number of possible data of length $N$, and decoding is possible if the total possible data is greater than the data that can be generated by substitution of the typical data $T > S k$. 

For our problem, the data can be modelled by a co-occurrence matrix $\cc$, where each data point is a bigram corresponding to an entry in the matrix.
Here $H_0 = \log(V^2)$ and $H(V)$ can be estimated from actual data in $\cc$.
Calculating this on en-wiki gave $N \approx \frac{V \log (V)}{\log(V^2) - H(V)} \leq 1.5V$,
meaning that little data is needed.
The solution requires solving
\begin{align}
    \max_{\pi} \log P(\pi(\cc)_{ij}) = \sum_{ij} \pi(\cc)_{ij} \log p_{ij}
    \label{eq:lhobj}
\end{align}
where $\pi$ is a permutation over $[V]$ and $\pi(\cc)$ applies
the same permutation to both rows and columns of $\cc$,
and $p$ is the true probability of the language.

\subsection{Bilingual lexicon induction}
Bilingual lexicon induction can be formulated similarly to the word substitution cipher where one language is seen as a substitution cipher of another one.
Compared to an actual bigram model, this is more sensible under
the word window model since finer
syntactic structure is not as important
and longer context should in fact transfer across languages.
However, because the statistical change between languages is rather involved,
there may not be a solution that substitutes the source $\cc_1$ to the typical high probability set in the target $\cc_2$.
Still, we already know that bilingual lexicon induction is possible with zero or minimal supervision and \eqref{eq:lhobj} still seems reasonable even
if a good solution is not guaranteed.



\subsection{Better unsupervised initialization with counts}

The main finding of this section is that the co-occurence matrix $\cc$ performs significantly better than the commonly used fasttext for unsupervised initialization.
In the low data regime, these raw counts start getting signal with 20\% to 50\% the data that fasttext vector requires.
For the word-decipherment setting, this method can solve the problem nearly completely whereas
fasttext vector stays at low accuracy even with much more data.

\begin{lstlisting}[language=Python]
def count_vec(Co, dim, alpha=0.5):
    return power(Co[:, :dim], alpha)
    
def svd_vec(Co, dim, alpha=0.5, beta=1):
    u, s, _ = svd(power(Co, alpha))
    return u[:, :dim] * power(s[:dim], beta)
\end{lstlisting}

When stronger statistical assumptions hold as in deciphering, we find that an SVD-based initialization is better, but it did not generalize to the actual cross-lingual case.
\begin{algorithm}
\caption{singular vector alignment initialization method}\label{alg:svdinit}
\begin{algorithmic}
\State \textbf{Input}  $\cc^1, \cc^2$, \quad \textbf{Output} $M$
\State $X = \operatorname{vectorize}(\cc^1)$
\State $Z = \operatorname{vectorize}(\cc^2)$
\State $U_1, s_1 = \operatorname{svd}(X X^{\T})$
\State $U_2, s_2 = \operatorname{svd}(Z Z^{\T})$
\State align the arbitrary sign of $U_1$, $U_2$ so that $\diag(U_1^\T U_2) \approx 1$
\State $M = d(U_1, U_2)$
\end{algorithmic}
\end{algorithm}

\subsection{Likelihood based method}
From $c_{ij}$, we may estimate $p_i \in \Delta^K$
where $p_{ij}$ is the probability that $j$ appears in a window centered on word $i$. The maximum likelihood estimate is $p_{ij} = c_{ij} / \sum_j c_{ij}$.
The problem is to find corresponding words between a pair of languages given co-occurrences in both languages and possibly some known alignments.
What is the least amount of data required to be successful at cross-lingual alignment? A necessary condition is that the language can align to itself based on co-occurrences under iid conditions.
In actual multi-lingual alignment problem, there is domain and meaning shift in addition to the noise from sampling.
In this section, we establish the minimum amount of data required to achieve alignment through co-occurrence statistics.
The question is weather we can uniquely align a subword to itself while knowing the correct alignment of all other subwords. We should not hope for any success in multilingual alignment before the amount of data passes this threshold.

Bayes rule tells us when a match is likely to be correct given certain counts.
Let the co-occurence probability vectors be $p_1, p_2, \ldots, p_K \in \Delta^K$ for each of the $K$ words.
Let the count vector $c \sim \Mult(N, p) \in \mathbb{Z_+}^K$ be drawn from the multinomial distribution $p_i$ with probability $p(i)$.
Bayes rule gives the posterior probability that $p_i$ is the vector generating $c$
\begin{align}
p(i \mid c) = \frac{p(i) p(c \mid p_i)}{\sum_j p(j) p(c \mid p_j)}
\end{align}
where $\log p(c \mid p_j) = \sum_j c_j \log p_{ij}$.
We are confident of the solution when a particular word $i$ has a large posterior probability compared to any other words.
We want to find the sample size $N_i = |c| = \sum_j c_j$ that $p_i$ can be identified with high probability if $c \sim \Mult(N_i, p_i)$.

This depends on how easily $p$ can be confused with an alternative $q$.
So we are interested in finding a condition so that
$p(c \mid p) > p(c \mid q)$

\begin{align}
\log p(c \mid p) &= \sum_k c_k \log p_k \\
H(c) &= \log p(c \mid p) - \log p(c \mid q)
\end{align}

% We are able to identify the correct $p$ if
% $\log p(c \mid p) - \log p(c \mid q) > 0$
% Thus, we seek a sample size $N$ such that
% $\Pr[] \approx 1$
% for a sample $c \sim \Mult(N, p)$.
This is the likelihood ratio test for $p$ vs $q$,
with test statistics $H(c)$.

It is also easy to calculate or compute the power of this procedure under the assumption of multinomial data.
For instance, here is a second-order characterization of the sample size, let $\hat{p} = c / N$, then $\cov[\hat{p}] =\frac1{N} (\diag(p) - p^\T p)$
and $\hat{p} \approx p + x$ with $x \sim \sN(0, \cov[\hat{p}])$.
\begin{align}
\frac1{N} \log \frac{p(c \mid p)}{p(c \mid q)} &= \sum_k \hat{p}_k \log \frac{p_k}{q_k}  \\
&= \sum_k (p_k + x_k)  \log \frac{p_k}{q_k} \\
&= \KL{p}{q} + y 
\end{align}
with $\sigma^2_y = r^\T \frac1{N} (\diag(p) - p p^\T) r$ where $r_k = \log \frac{p_k}{q_k}$.
\begin{align}
N \sigma^2_y &= \sum_k p_k \log^2 \frac{p_k}{q_k} - \left( \sum_k p_k \log \frac{p_k}{q_k} \right)^2 \\
&= \sum_k p_k \log^2 \frac{p_k}{q_k} - \KL{p}{q}^2
\end{align}

Applying a Gaussian tail-bound shows that the failure chance is bounded by
$\Pr[ y < -D] \leq \exp(-\frac{ND^2}{2 \sigma^2_y}) = \delta$
or $ N > 2 \log(1/\delta) \sigma^2_y / D^2$.
These quantities can be computed from monolingual data.



\subsection{Unsupervised word translation}
The previous section establish the minimum amount of data required to make progress on a lexicon given known correspondences. In this section, we analyze the case of unaligned distributions.
In the unsupervised setting, we only have $p$ and $q$ as a set, instead of a matching vector. As a result, we cannot simply evaluate $\KL{p}{q}$.
We are still interested in the question if a sample $\hat{p}$ comes from $p$ or $q$.
One simple and currently used strategy is to sort everything and apply the previous method on $\sort(\hat{p})$, $\sort(p)$, $\sort(q)$.
With enough samples, this approach works. However, it is not correcting for sample size.

Consider
$\Pr[\sort(\hat{p}) \mid \sort(p)] = \sum_i \sort(\hat{p})_i \log \sort(p)_i$.
$\sort(\hat{p})_1$ is the relatively frequency of the most frequent element.
In expectation, $\E[\sort(\hat{p})_1]] > \sort(p)_1$
since less probable elements can be more frequent in a sample.
This effect is significant when the sample size is insufficient to preserve
the frequency order of samples.

We want to find vector $p'$ such that $\Pr[\sort(\hat{p}) \mid p']$ is high. Instead of $\sort(p)_i$, we consider a typical sample $c_n$ of size $n$ from $p$.
Let $\hat{p}_n = c_n / \sum_j c_j$.
We can use resampling to evaluate $\E[\sort(\hat{p}_n)]$. 


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> svds.tex <==
% symbols to use
% X, Y are the embeddings, not ideal, but following existing work
% S_{XY} is the similarity matrix?
% what are the anchors

Bilingual lexicon induction is the task of matching up words in two different languages. We do some analysis on how similarity in co-occurrence structure of words in two different languages leads to matching vector spaces.


\section{Co-occurances and vectors}
The problem of supervised bilingual lexicon induction is to expand
the set of word translation given an initial anchor set.
Distributional methods and embedding space methods
have been proposed to tackle this problem.
The distributional method is directly based on the distributional hypothesis applied
across languages and early works \citep{rapp1995identifying, rapp1999automatic} in this domain are distributional methods.
Since the striking finding that embedding space
rotations gives good word translations,
there have been many successes using embedding space methods.

Concretely, let us consider the supervised lexicon induction where we start with some anchor
word pairs $A = [(x_i, y_i)]_{i=1}^a$.
where $x_i$ is a translation of $y_i$.

\paragraph{Distributional method.}
Distributional methods start with the 
monolingual word-word matrix $M_X, M_Y \in \R^{v \times a}$ where $v$ is the
vocabulary size and $a$ the size of some anchor set
that has correspondence across two languages.
Each row of $M$ represents a word, each column represents an anchor
that has a correspondence in the other language,
and each entry indicates the relationship between the word and the anchor.
This matrix represents the monolingual word-word co-occurence statistics.
The $v \times v$ cross-lingual similarity matrix is $C = M_X M_Y^\T$.

\paragraph{Embedding space method.}
Let $X, Y \in \R^{a \times p}$ be the matrix containing $a$ corresponding anchor embeddings
of dimension $p$ in two languages.
The embedding space methods proposes that there is a linear transform $W$ that allows us to map between the two spaces,
i.e. $Y \approx X W$.
For test word $\hat{x}$, we find $\hat{x} W$ and
then search for nearest neighbors in the embedding space of the other language.
Let $\Xh$ and $\Yh$ be the test embeddings as opposed to $X$, $Y$ the anchor embeddings.
The cross-lingual similarity matrix is $C = \Xh W \Yh^\T$.


\subsection{Equivalence}
We show that common embedding space method has a corresponding distributional space method.
Consider the cross-lingual similarity matrix for the anchors
$X W Y^\T$.
The transformation minimizing $||Y - XW||_2$ is $W = \minv{(X^\T X)} X^\T Y$.
Note that the rows of $X, Y \in \R^{a \times p}$ represent corresponding anchors.
We will use $\hat{X} \in \R^{v \times p}, \hat{Y} \in \R^{v' \times p}$ for the matrices
whose rows correspond to 
other vocabularies which we want to match.
The corresponding similarity matrix between the vocabulary represented by
$\Xh$ and $\Yh$ is
\begin{equation}
    C = \Xh \minv{(X^\T X)} X^\T \ Y \Yh^\T.
    \label{eq:emb_sim}
\end{equation}

The distribution method requires the monolingual similarity matrices $M_X$ and $M_Y$.
Suppose we construct the distributional matrix from embeddings as well so that: $M_\Xh = \Xh X^\T$
or $M_{ij} = x_i \cdot x_j$.
Then the cross-lingual similarity matrix is
\begin{equation}
    C' \eqdef M_\Xh M_\Yh^\T = \Xh  X^\T \ Y \Yh^\T. 
    \label{eq:dist_sim}
\end{equation}

By contrasting \eqref{eq:dist_sim} and \eqref{eq:emb_sim}, we can see
that the embedding space method \eqref{eq:emb_sim} has an extra whitening operation applied to $M_X$ where the inverse covariance matrix
$\minv{(X^\T X)} \in \R^{p \times p}$ appears, which is a whitening operation in the embedding space.

In a distributional space method,
instead of the embedding matrix $X$ and $Y$,
we have the distributional matrices $\Xh X^\T$ and $\Yh Y^\T$.
A matrix identity allows us to achieve the same whitening operation without
the need for an explict embedding space.
We can derive this by decomposing \eqref{eq:emb_sim} using SVD
where $X = U S V^\T$ and $\Xh = \Uh \Sh \Vh^\T$,
\begin{align}
M_\Xh = \Xh X^\T &= \Uh \Sh \Vh^\T V S U^\T,
\\ M_X = X X^\T &= U S^2 U^\T.
\end{align}

\begin{align}
   \Xh \minv{(X^\T X)} X^\T &= \Uh \Sh \Vh^\T \ V S^{-2} V^\T \ V S U^\T 
  \\ &= \Uh \Sh \Vh^\T \ V S^{-1} U^\T \label{eq:XXT_norm}
  \\ &= \Uh \Sh \Vh^\T \ V S U^\T \ U S^{-2} U^\T
  \\ &= \Xh X^\T U S^{-2} U^\T
  \\ &= \Xh X^\T {(X X^\T)^\dagger}
  \\ &= M_\Xh M_X^\dagger
\end{align}

Thus, finding the least square linear transform in the embedding space is equivalent to
Thus, finding the least square linear transform in the embedding space is equivalent to
dividing by $M_X$ in the distribution space before matching by dot products.
\begin{align}
    C &= \Xh \minv{(X^\T X)} X^\T \ Y \Yh^\T
    \\ &= \Xh X^\T \ \minv{(X^\T X)} \ Y \Yh^\T
    \\ &=  M_\Xh M_X^\dagger M_\Yh^\T.
\end{align}


Interestingly, while the embedding space transform $W = \minv{(X^\T X)} X^\T Y$ depends on anchor vectors for both languages,
the distributional method does a normalization in one language without considering the other space
i.e.  $Z_X = \Xh \minv{(X^\T X)} X^\T$ is not a function of $Y$.
The asymmetry is because we used the least squares solution in the embedding space, which is not symmetric.

The effect in the embedding space is whitening, 
this imposes a self-consistency requirement in the distribution space.
If we take the distributional vectors $m_i \in \R^a$
and measure its similarity with other words
$j \in \{1, \ldots, a\}$ by the inner product,
then the self-consistency of the distributional vectors means that $m_{ij} = m_i \cdot m_j$
and follows from properties of the pseudoinverse
\begin{align}
 \Zh Z^\T = \Mh M^\dagger M M^\dagger = \Mh M^\dagger = \Zh.
\end{align}


\section{Unsupervised induction}
Some popular unsupervised lexicon induction methods take advantage of both viewpoints.
\citet{artetxe2018robust} use a modified distributional vectors to initialize an iterative procedure in the embedding space
whereas \citet{alvarezmelis2018gromov} works in the distributional space only.
The corresponding distribution space used in \citet{artetxe2018robust}
is the symmetrized $M_X M_X^{-1/2}  = X X^\T (X X^\T)^{-1/2}$ and $M_Y M_Y^{-1/2}$.
\cite{alvarezmelis2018gromov} directly uses $M_X$ and $M_Y$.

\section{Related works}
\cite{smith2017offline}
\cite{rapp1999automatic}
\cite{rapp1995identifying}
\cite{artetxe2018robust}
\cite{alvarezmelis2018gromov}
